Controlled Automatic Task-Specific Synthetic Data Generation for Hallucination Detection

We present a novel approach to automatically generate non-trivial task-specific synthetic datasets for hallucination detection. Our approach features a two-step generation-selection pipeline, using hallucination pattern guidance and a language style alignment during generation. Hallucination pattern guidance leverages the most important task-specific hallucination patterns while language style alignment aligns the style of the synthetic dataset with benchmark text. To obtain robust supervised detectors from synthetic datasets, we also adopt a data mixture strategy to improve performance robustness and generalization. Our results on three datasets show that our generated hallucination text is more closely aligned with non-hallucinated text versus baselines, to train hallucination detectors with better generalization. Our hallucination detectors trained on synthetic datasets outperform in-context-learning (ICL)-based detectors by a large margin of 32%. Our extensive experiments confirm the benefits of our approach with cross-task and cross-generator generalization. Our data-mixture-based training further improves the generalization and robustness of hallucination detection.

==> table_external_submission/ablation_haleval.tex <==
\begin{table}[h]
\centering
\footnotesize
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
&  \multicolumn{4}{c}{Train Set}   \\
Test Set        & Ours    & Ours (w/o HPG) &  SimPrompt & HalEval &  Ave  \\
\midrule
\multicolumn{4}{l}{\textit{OpenDialKG}}   \\
 % \midrule
 Ours           &  0.920  & 0.852          & 0.911      &  0.646  & 0.832  \\
 % Ours (w/o HPG) &  0.946  &  0.976         & 0.944      &  0.659  & 0.881  \\
 SimPrompt      &  0.914  &  0.845         & 0.945      &  0.643  & 0.837  \\
 HalEval        &  0.850  &  0.861         & 0.849      &  0.994  & 0.889  \\
\midrule
\multicolumn{4}{l}{\textit{ReDial}}   \\
% \midrule
% &  \multicolumn{4}{c}{Train Set}   &
% Test Set  & LSA & HPG & w/o LSA & w/o HPG & Ave &
 % \midrule
 Ours           &   0.932  &  0.839        &   0.922     &  0.905  & 0.900   \\
 % Ours (w/o HPG) &   0.982 &   0.993         &  0.973      &  0.964  & 0.978   \\
 SimPrompt      &   0.932 & 0.822         &  0.945        &  0.921  & 0.905  \\
 HalEval        &   0.842 &   0.812       &  0.858      &  0.949 & 0.865 \\
\midrule
\multicolumn{4}{l}{\textit{SalesBot}}   \\
% \midrule
% &  \multicolumn{4}{c}{Train Set}   &
% Test Set  & LSA & HPG & w/o LSA & w/o HPG & Ave &
 % \midrule
 Ours           & 0.963  & 0.878        &  0.956        & 0.938  &  0.934  \\
 % Ours (w/o HPG) & 0.978  & 0.988        &  0.975        & 0.982  & 0.981 \\
 SimPrompt      & 0.975  & 0.898        &   0.977       & 0.956  &  0.952  \\
  HalEval       & 0.865  & 0.900        &  0.895        & 0.969  & 0.907 \\
\midrule
Ave             & 0.925  & 0.889        & 0.929         & 0.877  & 0.905 \\
\bottomrule
\end{tabular}}
\vspace{-10pt}
\caption{\small Ablation study. 
Column names denote the generation setup for train datasets and row names denote the setup for test datasets.
% This table reports the detector performance trained and evaluated on datasets generated with different modules. Column names denote the pipeline setup used to generate training datasets, and row names represent the pipeline setup for test datasets. 
}
\vspace{-15pt}
\label{table:ablation-v2}
\end{table}


==> table_external_submission/cross_model_generalization.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular*}{0.49\textwidth}{@{\extracolsep{\fill}}lcccc}
\toprule
& IG (Mean)  & OG Mean & Gap ($\Delta$) &  OG Std \\
\midrule
\multicolumn{4}{l}{\textit{OpenDialKG}} \\
Vanilla & \textbf{0.920} & 0.813 & -0.107  & 0.122  \\
Mixture & 0.908 & \textbf{0.859} & \textbf{-0.048}   & \textbf{0.079} \\
\midrule
\multicolumn{4}{l}{\textit{ReDial}} \\
Vanilla & \textbf{0.932} & 0.830 & -0.102  & 0.090 \\
Mixture & 0.913 & \textbf{0.869} & \textbf{-0.044}   & \textbf{0.063} \\
\midrule
\multicolumn{4}{l}{\textit{SalesBot}} \\
Vanilla & \textbf{0.963} & 0.895 & -0.068  & 0.073 \\
Mixture & 0.950 & \textbf{0.907} & \textbf{-0.042}   & \textbf{0.054} \\
\bottomrule
\end{tabular*}
\vspace{-6pt}
\caption{{\small Cross-generator generalization. 
% This table reports supervised detectors' performance on the test dataset generated by the same generator as its training data (In-Generator) and by other generators (Out-of-Generator).
% $\Delta$ is the performance gap between in-generator (IG) performance and out-of-generator (OG) performance. OG Std is the performance standard deviation on out-of-generator datasets. 
% Reported are based on F1 scores. Bold are preferred performance. 
}}
\vspace{-15pt}
\label{tab:robustness}
\end{table}





==> table_external_submission/cross_model_generalization_haleval.tex <==
\begin{table*}[t]
\centering
\footnotesize
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
& IG (Ours)  & OG (Ours) & Gap ($\Delta$) &  OG Std & IG (HalEavl) & OG (HalEval) & Gap & Std\\
\midrule
\multicolumn{4}{l}{\textit{OpenDialKG}} \\
Vanilla & \textbf{0.920} & 0.813 & -0.107  & 0.122  \\
Mixture & 0.908 & \textbf{0.859} & \textbf{-0.048}   & \textbf{0.079} \\
HalEval & \\
\midrule
\multicolumn{4}{l}{\textit{ReDial}} \\
Vanilla & \textbf{0.932} & 0.830 & -0.102  & 0.090 \\
Mixture & 0.913 & \textbf{0.869} & \textbf{-0.044}   & \textbf{0.063} \\
HalEval & \\
\midrule
\multicolumn{4}{l}{\textit{SalesBot}} \\
Vanilla & \textbf{0.963} & 0.895 & -0.068  & 0.073 \\
Mixture & 0.950 & \textbf{0.907} & \textbf{-0.042}   & \textbf{0.054} \\
HalEval & \\
\bottomrule
\end{tabular}
}
\vspace{-6pt}
\caption{{\small Cross-generator generalization. 
% This table reports supervised detectors' performance on the test dataset generated by the same generator as its training data (In-Generator) and by other generators (Out-of-Generator).
% $\Delta$ is the performance gap between in-generator (IG) performance and out-of-generator (OG) performance. OG Std is the performance standard deviation on out-of-generator datasets. 
% Reported are based on F1 scores. Bold are preferred performance. 
}}
\vspace{-15pt}
\label{tab:robustness}
\end{table*}



==> table_external_submission/cross_pattern_generalization.tex <==
\begin{table}[t]
\centering
\footnotesize
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
& Enty Incon. & Non. Resp. & Irre. Cont. & Overall \\
\midrule
\multicolumn{5}{l}{\textit{OpenDialKG}} \\
 Vanilla IP & 0.858 & 0.932 & 0.947 & 0.920 \\
 Vanilla OP & 0.451 & 0.932 & 0.931 & 0.771 \\
 Mixture IP & 0.829 & 0.931 & 0.948 & 0.908 \\ 
 Mixture OP & 0.762 & 0.865 & 0.896 & 0.841 \\
\midrule
\multicolumn{5}{l}{\textit{ReDial}} \\
 Vanilla IP & 0.849 & 0.969 & 0.975 & 0.932 \\
 Vanilla OP & 0.719 & 0.965 & 0.951 & 0.879 \\
 Mixture IP & 0.793 & 0.957 & 0.966 & 0.913 \\ 
 Mixture OP & 0.773 & 0.917 & 0.94 & 0.877 \\
\midrule
\multicolumn{5}{l}{\textit{SalesBot}} \\
 Vanilla IP & 0.932 & 0.978 & 0.987 & 0.963  \\
 Vanilla OP & 0.751 & 0.975 & 0.977 & 0.901 \\
 Mixture IP & 0.904 & 0.973 & 0.984 & 0.950 \\
 Mixture OP & 0.822 & 0.935 & 0.949 & 0.902 \\
\bottomrule
\end{tabular}
}
\vspace{-6pt}
\caption{{\small Out-of-pattern Performance. Column names denote the unseen patterns. 
% Cross-pattern generalization. This table compares the performances on hallucination patterns when they are seen and unseen. For rows of In-Pattern, the patterns in columns are included in the training data but are excluded for rows of Out-of-Pattern (Out-of-Ptn). Reported are average F1 scores across detectors.
}}
\label{tab:cross_pattern_generalization}
\end{table}

==> table_external_submission/cross_task_generalization.tex <==
\begin{table}[h]
\centering
\footnotesize

\resizebox{0.49\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
& \multicolumn{4}{c}{Train Set} \\
% \midrule
Test Set & OpenDialKG & ReDial & SalesBot & Ave \\
\midrule
% \multicolumn{5}{l}{\textit{Vanilla}}\\
% OpenDialKG & 0.920 & 0.869 & 0.874 & 0.888 \\
% ReDial     & 0.887 & 0.932 & 0.830 & 0.883 \\
% SalesBot   & 0.863 & 0.878 & 0.963 & 0.901 \\
% \midrule
% \multicolumn{5}{l}{\textit{Mixture}} \\
% OpenDialKG & 0.908 & 0.876 & 0.862 & 0.882 \\
% ReDial     & 0.884 & 0.913 & 0.823 & 0.873\\
% SalesBot   & 0.816 & 0.883 & 0.950 & 0.883\\


% \multicolumn{5}{l}{\textit{Vanilla}}\\
% OpenDialKG & -     & 0.869 & 0.874 & 0.872 \\
% ReDial     & 0.887 & -     & 0.830 & 0.859 \\
% SalesBot   & 0.863 & 0.878 & -     & 0.871 \\
% \midrule
% \multicolumn{5}{l}{\textit{Mixture}} \\
% OpenDialKG & -     & 0.876 & 0.862 & 0.869 \\
% ReDial     & 0.884 & -     & 0.823 & 0.854\\
% SalesBot   & 0.816 & 0.883 & -     & 0.850\\
% \midrule
% \multicolumn{5}{l}{\textit{HaluEval}} \\
% OpenDialKG & -     & 0.781 & 0.860 & 0.821  \\
% ReDial     & 0.638 & -     & 0.825  & 0.732 \\
% SalesBot   & 0.639 & 0.779 & -     & 0.709\\

\multicolumn{5}{l}{\textit{OpenDialKG}}\\
Vanilla & -     & 0.869 & 0.874 & \textbf{0.872} \\
Mixture & -     & 0.876 & 0.862 & \underline{0.869} \\
SimPrompt  & -  & 0.860 &  0.824 & 0.842 \\
HaluEval & -     & 0.781 & 0.860 & 0.821  \\
\midrule
\multicolumn{5}{l}{\textit{ReDial}} \\
Vanilla     & 0.887 & -     & 0.830 & \textbf{0.859} \\
Mixture     & 0.884 & -     & 0.823 & \underline{0.854}\\
SimPrompt & 0.842 & - & 0.783 & 0.813 \\
HaluEval     & 0.638 & -     & 0.825  & 0.732 \\

\midrule
\multicolumn{5}{l}{\textit{SalesBot}} \\
Vanilla   & 0.863 & 0.878 & -     & \textbf{0.871} \\
Mixture   & 0.816 & {0.883} & -     & \underline{0.850}\\
SimPrompt & 0.800 & 0.836 & - & 0.818 \\
HaluEval   & 0.639 & 0.779 & -     & 0.709\\

\bottomrule
\end{tabular}
}
\vspace{-6pt}
\caption{{\small Out-of-Task generalization. Column names denote the train benchmark and row names denote test benchmark. \textbf{Bold} indicate best in class and \underline{underline} signals the second. 
% This table reports the average detector performance trained and evaluated on different benchmark tasks. Column names denote the task of training dataset, and row names represent the task of testing dataset. Train and test datasets are generated by same LLMs. Reported are average F1 scores over the datasets generated by six LLM generators. 
}}
\vspace{-15pt}
\label{tab:cross_task_generalization}
\end{table}
